Ising-based Consensus Clustering on Specialized Hardware

The emergence of specialized optimization hardware such as CMOS annealers and adiabatic quantum computers carries the promise of solving hard combinatorial optimization problems more efficiently in hardware. Recent work has focused on formulating different combinatorial optimization problems as Ising models, the core mathematical abstraction used by a large number of these hardware platforms, and evaluating the performance of these models when solved on specialized hardware. An interesting area of application is data mining, where combinatorial optimization problems underlie many core tasks. In this work, we focus on consensus clustering (clustering aggregation), an important combinatorial problem that has received much attention over the last two decades. We present two Ising models for consensus clustering and evaluate them using the Fujitsu Digital Annealer, a quantum-inspired CMOS annealer. Our empirical evaluation shows that our approach outperforms existing techniques and is a promising direction for future research.

==> alt.tex <==
\appendix

\section{Alternate Pairwise Similarity-Based Ising Model}

Consider a cluster numbered $c$, whose binary representation is $ c_l ... c_0 $, where $l = [\log k_{\pi^*}]$.
For each data point $u \in X$, and for each $i \in [0, l]$, we initially set variables $q_{ui}$ to 0. If $\pi^*$ assigns $u$ to cluster $c$ and $c_i =1$ we set $q_{ui} = 1$. So essentially for any point $u$, the bit sequence $q_{ul} ... q_{u0}$ would give the binary expansion of the cluster number it belongs to. \added[id=ar]{There is no need for a one-hot encoding anymore.}

The sum of quadratic terms  $\sum_{i=1}^{l}  (q_{ui} - q_{vi})^2 $ is 0 iff $\pi^*$ assigns both $u, v \in X$ to the same cluster. Therefore the value
\begin{equation}
\sum_{\substack{u, v \in X: \\ \pi^*(u) = \pi^*(v)}} (1 - S_{uv}) = \sum_{u, v \in X} (1-S_{uv})
\sum_{i=1}^{l}  (q_{ui} - q_{vi})^2
\label{eq:alt-obj}
\end{equation}
and represents the sum of within-cluster dissimilarities resulting from $\pi^*$.
 In particular, the value $(1-S_{uv})$ is the fraction of the clusterings in $\Pi$ that assign $u$ and $v$ to different clusters while $\pi^*$ assigns them to the same cluster. Hence, we seek a consensus clustering $\pi^*$ that minimizes this value. %This optimization problem can easily be reformulated to the following QUBO:
 We therefore reformulate the optimization problem in Equation (\ref{eq:sim_based}) as QUBO:
\begin{equation}
\begin{aligned}
\min \sum_{u, v \in X} (1-S_{uv})
\sum_{c=1}^{K}  q_{uc} q_{vc} + \sum_{u \in X} A (\sum_{c=1}^{K} q_{uc} -1)^2. \label{eq:ising_cluster} 
\end{aligned}
\end{equation}
where the term $ \sum_{u \in X} A (\sum_{k=1}^{k_{\pi^*}} q_{uk} -1)^2$ is added to the objective function to ensure that the constraints (\ref{eq:one_hot}) are satisfied. The value $A$ is positive constant that penalizes the objective value whenever the constraints (\ref{eq:one_hot}) are violated.  One can show that if $A \geq n$, then the optimal solution of the QUBO defined in Equation (\ref{eq:ising_cluster}) does not violate the constraints (\ref{eq:one_hot}). We omit the proof and refer readers to \cite{kumar2018quantum} for a similar type of result.


%{\color{red}
%\added[id=hm]{COMMENT: red text below rewritten above}

%To model the pairwise similarity-based approach as a QUBO, we modify the standard clustering Ising model \cite{kumar2018quantum} to use use distances that are based on the pairwise similarity consensus matrix:
%\added[id=am]{Refer to the equation where $S_{ij}$'s are initially defined}
% \begin{equation}
% \begin{aligned}
% E(q) = \sum_{i<j} (1-S_{ij})
% \sum_{k=1}^{K^*}  q_k^i q_k^j + \sum_{i=1}^n w (\sum_{k=1}^{K^*} q_k^i -1)^2. \label{eq:ising_cluster} 
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
% E(\textbf{q}) = \sum_{u, v \in X} (1-S_{uv})
% \sum_{k=1}^{k_{\pi^*}}  q_{uk} q_{vk} + \sum_{u \in X} w (\sum_{k=1}^{k_{\pi^*}} q_{uk} -1)^2. %\label{eq:ising_cluster} 
% \end{aligned}
% \end{equation}
% %\added[id=hm]{COMMENT: Use $q_{ik}$ instead of $q_{k}^i$}\\
% %\added[id=ec]{COMMENT: Note that the $q_k^i$ notation follows the existing QUBO formulation for clustering \url{https://arxiv.org/pdf/1708.05753.pdf} \cite{kumar2018quantum}}
% %\added[id=am]{I prefer $q_{ik}$, my usual interpretation is superscript means exponential}

% In this formulation, the consensus partition is represented using one-hot encoding, i.e., $k_{\pi^*}$ binary variables $q_{uk}$ such that $q_{uk} = 1 \iff $ \replaced[id=hm]{$\pi^*(u) = k$ }{$x_i {\in} S_k$}. The terms %$\sum_{i<j} (1-S_{ij}) \sum_{k=1}^K  q_k^i q_k^j$
% $\sum_{u, v \in X} (1-S_{uv})
% \sum_{k=1}^{k_{\pi^*}} q_{uk} q_{vk} $ represent the sum of within-cluster dissimilarities. $1-S_{uv}$ is the dissimilarity between $u, v \in X$, i.e., the fraction of partitions that \emph{disagree} on the clustering of points $u$ and $v$.\footnote{Note that minimizing the within-cluster dissimilarity is equivalent to maximizing the within-cluster similarity. In clustering algorithms, we often use dissimilarities (e.g., distances) rather than similarities.} As each point is assigned to exactly one cluster, the above QUBO model includes the quadratic penalty terms % $\sum_{i=1}^n w (\sum_{k=1}^K q_k^i -1)^2$ 
% $\sum_{u \in X} w (\sum_{k=1}^{k_{\pi^*}} q_{uk} -1)^2$ that ensure that the one-hot encoding holds: If $u \in X$ is assigned to exactly one cluster %$(\sum_{k=1}^K q_k^i -1)^2 = 0$, 
% $w (\sum_{k=1}^{k_{\pi^*}} q_{uk} -1)^2$ otherwise %the term evaluates to a positive and 
% the objective is penalized for violating the one-hot encoding constraint with the penalty being weighted by $w$. We can show that setting $w=n$ guarantees that the one-hot encoding holds and the optimal solution is feasible. We omit the proof and refer readers to \cite{kumar2018quantum} for a similar type of result.
% }
